Flow-Level Packet Loss Detection via Sketch Decomposition and Matrix Optimization

For cloud service providers, fine-grained packet loss detection across data centers is crucial in improving their service level and increasing business income. However, the inability to obtain sufficient measurements makes it difficult owing to the fundamental limit that the wide-area network links responsible for communication are not under their management. Moreover, millisecond-level delay jitter and clock synchronization errors in the WAN disable many tools that perform well in data center networks on this issue. Therefore, there is an urgent need to develop a new tool or method. In this work, we propose SketchDecomp, a novel loss detection method, from a mathematical perspective that has never been considered before. Its key is to decompose sketches upstream and downstream into several sub-sketches and builds a low-rank matrix optimization model to solve them. Extensive experiments on the test bed demonstrate its superiority.

==> data/Abstract.tex <==
\

==> data/Preliminaries.tex <==
% \section{Preliminaries}

% \subsection{Count-min Sketch}
% The count-min sketch (CM-Sketch) is a particular data structure to count and record the frequency of each element of a flow, with a certain confidence level. Unlike traditional hash tables, it utilizes multiple, say $d$, mutually independent hash functions $\{h_i\}_{i=1}^d$ to against the overcounting  caused by collisions. Basically, CM-Sketch is a $w \times d$ matrix denoted as $C$, whose $i$-th row is the count created by $h_i$. 
% In the beginning, The matrix is initialized to all zero. For each incoming element $a$, we hash it in turn by $\{h_i\}_{i=1}^d$ to get $d$ column indexes and then increase the value of the matrix $C(i,h_i(a))$ at the respective index by one, as shown in Figure \ref{fig:sketch}. After all flow elements have been viewed, The matrix will keep fixed and enable querying. The rule for querying is concise: The final estimated count of an element $a$ is the least value of the counts given by all hash functions, i.e., $\min_i h_i(a)$. 

% \begin{figure}
%     \centering
%    \includegraphics[width=0.5\linewidth]{figure/sketch.pdf}
%     \caption{Sketch}
%     \label{fig:sketch}
% \end{figure}
% \subsection{Paket lo }
